MLI-NeRF: Multi-Light Intrinsic-Aware Neural Radiance Fields

Current methods for extracting intrinsic image components, such as reflectance and shading, primarily rely on statistical priors. These methods focus mainly on simple synthetic scenes and isolated objects and struggle to perform well on challenging real-world data. To address this issue, we propose MLI-NeRF, which integrates \textbf{M}ultiple \textbf{L}ight information in \textbf{I}ntrinsic-aware \textbf{Ne}ural \textbf{R}adiance \textbf{F}ields. By leveraging scene information provided by different light source positions complementing the multi-view information, we generate pseudo-label images for reflectance and shading to guide intrinsic image decomposition without the need for ground truth data. Our method introduces straightforward supervision for intrinsic component separation and ensures robustness across diverse scene types. We validate our approach on both synthetic and real-world datasets, outperforming existing state-of-the-art methods. Additionally, we demonstrate its applicability to various image editing tasks. The code and data are publicly available.

==> teaser.tex <==

\centering
\includegraphics[width=1.0\linewidth]{pic/first_pic-cropped.pdf}
\vspace{-7mm}
\captionof{figure}{Given real-world images from ReNe dataset \cite{Toschi_2023_CVPR} (a), our method learns the neural radiance fields that enable novel view synthesis and relighting (b), and intrinsic decomposition (c) simultaneously. Image editing applications (d) can also be employed, such as reflectance editing, reflectance editing plus relighting or shading editing (simulating two lights).}
\label{teaser}
\vspace{3mm}

